Attention: Not Just Another Dataset for Patch-Correctness Checking

Automated Program Repair (APR) techniques have drawn wide attention from both academia and industry. Meanwhile, one main limitation with the current state-of-the-art APR tools is that patches passing all the original tests are not necessarily the correct ones wanted by developers, i.e., the plausible patch problem. To date, various Patch-Correctness Checking (PCC) techniques have been proposed to address this important issue. However, they are only evaluated on very limited datasets as the APR tools used for generating such patches can only explore a small subset of the search space of possible patches, posing serious threats to external validity to existing PCC studies. In this paper, we construct an extensive PCC dataset (the largest manually labeled PCC dataset to our knowledge) to revisit all state-of-the-art PCC techniques. More specifically, our PCC dataset includes 1,988 patches generated from the recent PraPR APR tool, which leverages highly-optimized bytecode-level patch executions and can exhaustively explore all possible plausible patches within its large predefined search space (including well-known fixing patterns from various prior APR tools). Our extensive study of representative PCC techniques on the new dataset has revealed various surprising findings and provided guidelines for future PCC research.

==> Raw-data/literature_review.tex <==
\begin{table*}[htb]
	\centering
	\small
	\renewcommand{\arraystretch}{1.0}
    \setlength{\tabcolsep}{3pt}
	\caption{Datasets used in existing \pcc{} work}\label{table:revisit}
	\begin{adjustbox}{width=2.0\columnwidth}
	\begin{tabular}{c|c|c|c|c|c|c}
	\toprule
	\multirow{2}{*}{\textbf{Work}} & 	\multirow{2}{*}{\textbf{Studied technique}} & 	\multirow{2}{*}{\textbf{Scale}} & 	\multirow{2}{*}{\textbf{Ratio}} & 	\multicolumn{3}{c}{\textbf{Dataset source}}  \\ \cline{5-7}
	
	&&& (correct/overfitting)& \textbf{Subject source} & \textbf{Patch source} & 	\textbf{Early stop}\\ \hline
	
Tan~\etal{}~\cite{Tan2016anti} & \tabincell{c}{\antipattern{}} & 289 & 30/259 & CoREBench~\cite{bohme2014corebench}, GenProg~\cite{le2012genprog} &
\tabincell{c}{\textbf{ All from APR tools} \\ GenProg, mGenProg~\cite{Tan2016anti}, SPR~\cite{long2015staged}, mSPR~\cite{Tan2016anti}} & 4/4 \\ \hline
	
	Le~\etal{}~\cite{le2017s3} & \tabincell{c}{\sthree{}} & 85 & 25/60 & \tabincell{c}{100 bugs from 62 subjects} \Comment{100 real world bugs}  &
\tabincell{c}{\textbf{All from APR tools} \\ \sthree{}, Enumerative~\cite{reynolds2015counterexample}, CVC4~\cite{reynolds2015counterexample}, Angelix~\cite{mechtaev2016angelix}} & 4/4 \\ \hline
	
	Yang~\etal{}~\cite{yang2017better} & \tabincell{c}{\opad{}} & 449 & 22/427 & \tabincell{c}{45 bugs from 7 subjects}  &
\tabincell{c}{\textbf{All from APR tools} \\ GenProg, AE~\cite{weimer2013leveraging}, Kali\cite{qi2015analysis}, and SPR} & 4/4 \\ \hline
	
	Xin~\etal{}~\cite{DBLP:conf/kbse/XinR17/ssfix} & \tabincell{c}{ \ssfix{}} & 153 & 122/31 & \tabincell{c}{\dfjold{} \\ \textit{exclude Mockito}}  &
	\tabincell{c}{\textbf{All from APR tools} \\ \ssfix{}, jGenProg, jKali~\cite{martinez2016astor}, Nopol, HDRepair~\cite{le2016history}, ACS} & 5/5 \\ \hline
	
	Xiong~\etal{}~\cite{xiong2018identifying} & \tabincell{c}{ \patchsim{}} & 139 & 29/110 & \tabincell{c}{\dfjold{} \\ \textit{exclude Closure, Mockito}}  &
	\tabincell{c}{\textbf{All from APR tools} \\ jGenPro~\cite{martinez2016astor}, Nopol~\cite{xuan2017nopol}, jKali, ACS~\cite{DBLP:conf/icse/XiongWYZH0017/acs}, HDRepair} & 5/5 \\ \hline
	
	Wen~\etal{}~\cite{DBLP:conf/icse/WenCWHC18} & \tabincell{c}{ CapGen~\cite{DBLP:conf/icse/WenCWHC18}} & 202 & 28/174 & \tabincell{c}{\dfjold{} \\ \textit{exclude Closure, Mockito}}  &
	\tabincell{c}{\textbf{All from APR tools} \\ CapGen} & 0/1 \\ \hline
	
	Xin~\etal{}~\cite{10.1109/GI.2019.00012} & \tabincell{c}{ sharpFix~\cite{xin2019revisiting}} & 82 & 56/26 & \tabincell{c}{Bugs.jar \\ \textit{127 bugs from 7 projects in Bugs.jar}}  &
	\tabincell{c}{\textbf{All from APR tools} \\ sharpFix, \ssfix{}~\cite{DBLP:conf/kbse/XinR17/ssfix}} & 2/2 \\ \hline
	
	Tian~\etal{}~\cite{tian2020evaluating} & \tabincell{c}{Embedding-based}& 1,000 & 468/532 & \dfjold{} &
	\tabincell{c}{\textbf{778 from APR tools} \\ RSRepair-A~\cite{yuan2018arja}, jKali, ACS, SimFix~\cite{jiang2018shaping}, TBar~\cite{liu2019tbar}, etc., 17 tools in total \\ \textbf{232 from developer patches} \\ *\textit{Supplemented to balance the dataset}} & 12/17 \\ \hline
	
	%Wang~\etal{}~\cite{} & \tabincell{c}{Static and dynamic, oracle required and not required techniques \\ PATCH-SIM, Opad, DiffTGen, Daikon, etc., 12 techniques in total}& 602 & 248:654 & \dfjold{} &\tabincell{c}{\textbf{All from APR tools} \\ jGenProg, DynaMoth, KPAR, SequencR, etc, 21 tools in total } & Y/N \\ 

	Wang~\etal{}~\cite{DBLP:conf/kbse/WangWLWQZMJ20} & \tabincell{c}{
	12 \pcc{} techniques}& 902 & 248/654 & \dfjold{} &
	\tabincell{c}{\textbf{All from APR tools} \\ jGenProg, DynaMoth~\cite{durieux2016dynamoth}, SequencR~\cite{chen2019sequencer}, etc., 21 tools in total } & 16/21 \\ 
	
	
	
	\bottomrule
	\end{tabular}
	\end{adjustbox}
\end{table*}

==> Tables/Patch_sim_dev.tex <==
\begin{tabular}{l|r|r|r|r|r}
\toprule
 & \textit{TP} & \textit{FP} & \textit{TN} & \textit{FN} & \textit{\correctrecall}\\
\midrule
\textit{developer patches} & 0 & 65 & 110 & 0 & 62.86\% \\
\bottomrule
\end{tabular}
\label{tab:patch_sim_dev}

==> Tables/anti_random_1.2.tex <==
\begin{tabular}{c|l|c|c|c|c|c}
\toprule
\multicolumn{2}{c|}{\textbf{Anti-pattern}}       & TP  & \textbf{FP} & \textbf{TN} & \textbf{FN} & \textbf{Precision} & \textbf{Recall} \\ \midrule
\multicolumn{2}{c|}{\textbf{Shangwen's   Paper}} & 219 & 37          & 211         & 435         & 85.50\%            & 33.49\%         \\
\multicolumn{2}{c|}{\textbf{Dataset 1.2}}        & 176 & 10          & 39          & 1132        & 94.62\%            & 13.46\%         \\
\multicolumn{2}{c|}{\textbf{Dataset 1.2-Random}} & 644 & 25          & 24          & 664         & 96.26\%            & 49.24\%        
\end{tabular}

==> Tables/anti_random_2.0.tex <==
\begin{tabular}{c|l|c|c|c|c|c}
\toprule
\textbf{Random   Select}    & TP  & \textbf{FP} & \textbf{TN} & \textbf{FN} & \textbf{Precision} & \textbf{Recall} \\ \midrule
\textbf{Shangwen's   Paper} & 219 & 37          & 211         & 435         & 85.50\%            & 33.49\%         \\
\textbf{Dataset 1.2}        & 644 & 25          & 24          & 664         & 96.26\%            & 49.24\%         \\
\textbf{Dataset 2.0}        & 305 & 18          & 18          & 336         & 94.43\%            & 47.58\%         \\
Dataset 1.2   \& 2.0        & 949 & 43          & 42          & 1000        & 95.67\%            & 48.69\%         \\ \bottomrule
\end{tabular}

==> Tables/anti_score_1.2.tex <==
\begin{tabular}{c|l|c|c|c|c|c}
\toprule
\multicolumn{2}{c|}{\textbf{Anti-pattern}}       & \textbf{FP} & \textbf{TN} & \textbf{FN} & \textbf{Precision} & \textbf{Recall} \\ \midrule
\multicolumn{2}{c|}{\textbf{Shangwen's   Paper}} & 37          & 211         & 435         & 85.50\%            & 33.49\%         \\
\multicolumn{2}{c|}{\textbf{Dataset 1.2}}        & 10          & 39          & 1132        & 94.62\%            & 13.46\%         \\
\multicolumn{2}{c|}{\textbf{Dataset 1.2-Random}} & 25          & 24          & 664         & 96.26\%            & 49.24\%   \\
\bottomrule
\end{tabular}

==> Tables/anti_score_2.0.tex <==
\begin{tabular}{c|l|c|c|c|c}
\toprule
\textbf{Anti-pattern}       & TP  & \textbf{FP} & \textbf{TN} & \textbf{FN} & \textbf{Precision} & \textbf{Recall} \\ \midrule
\textbf{Shangwen's   Paper} & 219 & 37          & 211         & 435         & 85.50\%            & 33.49\%         \\
\textbf{Dataset 1.2}        & 176 & 10          & 39          & 1132        & 94.62\%            & 13.46\%         \\
\textbf{Dataset 2.0}        & 187 & 18          & 18          & 453         & 91.22\%            & 29.17\%         \\
Dataset 1.2   \& 2.0        & 363 & 28          & 57          & 1585        & 92.84\%            & 18.63\%         \\ \bottomrule
\end{tabular}

==> Tables/capgen_performance.tex <==
% \begin{tabular}{l|r|r|r|r|r|r|r|r|r}
% \toprule
% CapGen & \textit{TP} & \textit{FP} & \textit{TN} & \textit{FN} & \textit{precision} & \textit{recall} & \textit{\correctrecall} & \textit{AUC} & \textit{AVR}\\
% \midrule
% \shangwendata & 510 & 144 & 104 & 144 & 77.98\% & 77.98\% & 41.94\% & 64.04\% & 2.14(9.1)\\
% \dfjoldprapr & 1,222 & 42 & 5 & 42 & 96.68\% & 96.68\% & 10.64\% & 47.80\% & 7.38(10.69)\\
% \dfjnewprapr & 1,827 & 78 & 5 & 78 & 95.91\% & 95.91\% & 6.02\% & 45.98\% & 6.62(9.64)\\
% \dfjmerge & 2,254 & 235 & 36 & 235 & 90.56\% & 90.56\% & 13.28\% & 50.34\% & 5.49(12.87)\\
% \dfjbalance & 128 & 143 & 128 & 143 & 47.23\% & 47.23\% & 47.23\% & 47.32\% & -\\
% \bottomrule
% \end{tabular}
% \label{tab:capgen_performance}


% \begin{tabular}{l|r|r|r|r|r|r|r|r|r}
% \toprule
% CapGen & \textit{TP} & \textit{FP} & \textit{TN} & \textit{FN} & \textit{precision} & \textit{recall} & \textit{\correctrecall} & \textit{AUC} & \textit{AVR}\\
% \midrule
% \shangwendata & 510 & 144 & 104 & 144 & 77.98\% & 77.98\% & 41.94\% & 64.04\% & 2.14(9.1)\\
% \dfjoldprapr & 1222 & 42 & 5 & 42 & 96.68\% & 96.68\% & 10.64\% & 47.80\% & 7.38(10.69)\\
% \dfjnewprapr & 1827 & 78 & 5 & 78 & 95.91\% & 95.91\% & 6.02\% & 45.98\% & 6.62(9.64)\\
% \dfjmerge & 2253 & 236 & 35 & 236 & 90.52\% & 90.52\% & 12.92\% & 50.34\% & 5.49(12.87)\\
% \dfjbalance & 133 & 138 & 133 & 138 & 49.08\% & 49.08\% & 49.08\% & 50.77\% & -\\
% \bottomrule
% \end{tabular}
% \label{tab:capgen_performance}

% \begin{tabular}{l|r|r|r|r|r|r|r|r|r}
% \toprule
% CapGen & \textit{TP} & \textit{FP} & \textit{TN} & \textit{FN} & \textit{precision} & \textit{recall} & \textit{\correctrecall} & \textit{PR-AUC} & \textit{AVR}\\
% \midrule
% \shangwendata & 510 & 144 & 104 & 144 & 77.98\% & 77.98\% & 41.94\% & 46.22\% & 2.14(9.1)\\
% \dfjoldprapr & 1222 & 42 & 5 & 42 & 96.68\% & 96.68\% & 10.64\% & 14,95\% & 7.38(10.69)\\
% \dfjnewprapr & 1827 & 78 & 5 & 78 & 95.91\% & 95.91\% & 6.02\% & 11.42\% & 6.62(9.64)\\
% \dfjmerge & 2253 & 236 & 35 & 236 & 90.52\% & 90.52\% & 12.92\% & 16.87\% & 5.49(12.87)\\
% \dfjbalance & 133 & 138 & 133 & 138 & 49.08\% & 49.08\% & 49.08\% & 54.75\% & -\\
% \bottomrule
% \end{tabular}
% \label{tab:capgen_performance}

\begin{tabular}{l|r|r|r|r|r|r|r|r|r}
\toprule
CapGen & \textit{TP} & \textit{FP} & \textit{TN} & \textit{FN} & \textit{\overfitprecision} & \textit{\overfitrecall} & \textit{\correctrecall} & \textit{\prauc} & \textit{\avr}\\
\midrule
\shangwendata & 510 & 144 & 104 & 144 & 78.0\% & 78.0\% & 41.9\% & 46.2\% & 2.1(9.1)\\
\dfjoldprapr & 1222 & 42 & 5 & 42 & 96.7\% & 96.7\% & 10.6\% & 14.9\% & 7.4(10.7)\\
\dfjnewprapr & 1827 & 78 & 5 & 78 & 95.9\% & 95.9\% & 6.0\% & 11.4\% & 6.6(9.6)\\
\dfjmerge & 2253 & 236 & 35 & 236 & 90.5\% & 90.5\% & 12.9\% & 16.9\% & 5.5(12.9)\\
\dfjbalance & 133 & 138 & 133 & 138 & 49.1\% & 49.1\% & 49.1\% & 54.8\% & -\\
\bottomrule
\end{tabular}
\label{tab:capgen_performance}

==> Tables/dataset_intro.tex <==
\begin{tabular}{@{}c|c|c|c@{}}
\toprule
\textbf{Category} & \textbf{Techniques} & \textbf{Datasets Used   to Evaluate}   & \textbf{Scale} \\ \midrule
\multirow{4}{*}{\textbf{Static}}  & S3                  & \begin{tabular}[c]{@{}c@{}}52 bugs in small programs, a subset of\\      the IntroClass benchmark translated to Java; 100 large real-world\\      Java bugs that we collected from GitHub\end{tabular} & 152            \\ \cmidrule(l){2-4} 
                                  & ssFix               & \begin{tabular}[c]{@{}c@{}}Defects4J\\      bug dataset (version 0.1.0)\end{tabular}                                                                                                                   & 357            \\ \cmidrule(l){2-4} 
                                  & CapGen              & Defects4j benchmark                                                                                                                                                                                    & 224            \\ \cmidrule(l){2-4} 
                                  & Anti-patterns       & \begin{tabular}[c]{@{}c@{}}49 defects from\\      the CoREBench benchmarks; \textgreater{}=37 defects from the\\      GenProg benchmarks\end{tabular}                                                  & 49             \\ \midrule
\multirow{2}{*}{\textbf{Dynamic}} & Opad                & \begin{tabular}[c]{@{}c@{}}45 bugs from 7 large systems (the same benchmark\\      used by GenProg and SPR)\end{tabular}                                                                               & 45             \\ \cmidrule(l){2-4} 
                                  & PATCH-SIM           & \begin{tabular}[c]{@{}c@{}}139 patches\\      generated from jGen-\\      Prog, Nopol, jKali, ACS and HDRepair\end{tabular}                                                                            & 139            \\ \midrule
\textbf{Learning Based}           & Embedding           & Liu et al, Xiong et al., Defects4j developers                                                                                                                                                          & 1000           \\ \bottomrule
\end{tabular}

==> Tables/embedding_score_1.2.tex <==
\begin{tabular}{c|l|c|c|c|c|c|c|c}
\toprule
\multicolumn{2}{c|}{\textbf{BERT-LR}}           & \textbf{Positive} & \textbf{Negative} & \textbf{Acc.} & \textbf{Prec.} & \textbf{Recall.} & \textbf{F1} & \textbf{AUC} \\ \midrule
\multicolumn{2}{c|}{\textbf{Embedding   paper}} & 468               & 532               & 74.4          & 73.8           & 70.3             & 72.0        & 0.808        \\
\multicolumn{2}{c|}{\textbf{Dataset 1.2}}     & 44                & 1092              & 79.4          & 8.7            & 45.5             & 14.6        & 0.699        \\
\multicolumn{2}{c|}{\textbf{Dataset 1.2-Random}}     & 49                & 1308              & 49.8          & 4.0            & 57.1             & /        & /        \\
\bottomrule
\end{tabular}

==> Tables/embedding_score_2.0.tex <==
\begin{tabular}{c|l|c|c|c|c|c|c|c}
\toprule
\multicolumn{2}{c|}{\textbf{BERT-LR}}           & \textbf{Positive} & \textbf{Negative} & \textbf{Acc.} & \textbf{Prec.} & \textbf{Recall.} & \textbf{F1} & \textbf{AUC} \\ \midrule
\multicolumn{2}{c|}{\textbf{Embedding   paper}} & 468               & 532               & 74.4          & 73.8           & 70.3             & 72.0        & 0.808        \\
\multicolumn{2}{c|}{\textbf{Dataset   1.2}}     & 44                & 1092              & 79.4          & 8.7            & 45.5             & 14.6        & 0.699        \\
\multicolumn{2}{c|}{\textbf{Dataset   2.0}}     & 34                & 604               & 69.0          & 6.4            & 35.3             & 10.8        & 0.599        \\
\multicolumn{2}{c|}{\textbf{Dataset   1.4}}     & 78                & 1696              & 75.6          & 7.7            & 41.0             & 12.9        & 0.660        \\
\multicolumn{2}{c|}{\textbf{Balanced Dataset}}  & 78                & 88                & 60.8          & 62.7           & 41               & 49.6        & 0.681        \\ \bottomrule
\end{tabular}

==> Tables/entropy_average.tex <==
\begin{tabular}{l|r|r|r|r|r}
\toprule
Mean Value & \textit{ssFix} & \textit{S3} & \textit{CapGen} & \textit{\sumentropy} & \textit{\meanentropy}\\
\midrule
\dfjnewprapr Correct & 1.52 & 10.60 & 0.37 & 30.76 & 3.15\\
\dfjnewprapr Overfitting & 1.56 & 15.73 & 0.41 & 39.72 & 3.17\\
\shangwendata Correct & 1.49 & 11.71 & 0.44 & 29.37 & 1.89\\
\shangwendata Overfitting & 1.35 & 26.35 & 0.25 & 44.14 & 3.80\\
Developer & 1.16 & 40.64 & 0.26 & 45.82 & 1.93\\
\bottomrule
\end{tabular}
\label{tab:entropy_average}

==> Tables/opad_correct_recall_dev_patches.tex <==
\begin{tabular}{l|r|r|r|r|r}
\toprule
 & \textit{TP} & \textit{FP} & \textit{TN} & \textit{FN} & \textit{\correctrecall}\\
\midrule
E-Opad & 0 & 111 & 685 & 0 & 86.06\%\\
R-Opad & 0 & 167 & 629 & 0 & 79.02\%\\
\bottomrule
\end{tabular}
\label{tab:opad_correct_recall_of_dev_patches}

==> Tables/s3_performance.tex <==
% \begin{tabular}{l|r|r|r|r|r|r|r|r|r}
% \toprule
% S3 & \textit{TP} & \textit{FP} & \textit{TN} & \textit{FN} & \textit{precision} & \textit{recall} & \textit{\correctrecall} & \textit{AUC} & \textit{AVR}\\
% \midrule
% \shangwendata & 517 & 137 & 111 & 137 & 79.05\% & 79.05\% & 44.76\% & 62.08\% & 2.80(9.1)\\
% \dfjoldprapr & 1,222 & 42 & 5 & 42 & 96.68\% & 96.68\% & 10.64\% & 53.56\% & 8.15(10.69)\\
% \dfjnewprapr & 1,826 & 79 & 4 & 79 & 95.85\% & 95.85\% & 4.82\% & 56.63\% & 7.15(9.64)\\
% \dfjmerge & 2,248 & 241 & 30 & 241 & 90.32\% & 90.32\% & 11.07\% & 45.03\% & 7.00(12.87)\\
% \dfjbalance & 121 & 150 & 121 & 150 & 44.65\% & 44.65\% & 44.65\% & 45.77\% & -\\
% \bottomrule
% \end{tabular}
% \label{tab:s3_performance}

% \begin{tabular}{l|r|r|r|r|r|r|r|r|r}
% \toprule
% S3 & \textit{TP} & \textit{FP} & \textit{TN} & \textit{FN} & \textit{precision} & \textit{recall} & \textit{\correctrecall} & \textit{AUC} & \textit{AVR}\\
% \midrule
% \shangwendata & 517 & 137 & 111 & 137 & 79.05\% & 79.05\% & 44.76\% & 61.57\% & 2.8(9.1)\\
% \dfjoldprapr & 1222 & 42 & 5 & 42 & 96.68\% & 96.68\% & 10.64\% & 53.56\% & 8.15(10.69)\\
% \dfjnewprapr & 1826 & 79 & 4 & 79 & 95.85\% & 95.85\% & 4.82\% & 56.63\% & 7.15(9.64)\\
% \dfjmerge & 2250 & 239 & 32 & 239 & 90.40\% & 90.40\% & 11.81\% & 45.03\% & 7(12.87)\\
% \dfjbalance & 120 & 151 & 120 & 151 & 44.28\% & 44.28\% & 44.28\% & 44.57\% & -\\
% \bottomrule
% \end{tabular}
% \label{tab:s3_performance}

% \begin{tabular}{l|r|r|r|r|r|r|r|r|r}
% \toprule
% S3 & \textit{TP} & \textit{FP} & \textit{TN} & \textit{FN} & \textit{precision} & \textit{recall} & \textit{\correctrecall} & \textit{PR-AUC} & \textit{AVR}\\
% \midrule
% \shangwendata & 517 & 137 & 111 & 137 & 79.05\% & 79.05\% & 44.76\% & 45.32\% & 2.8(9.1)\\
% \dfjoldprapr & 1222 & 42 & 5 & 42 & 96.68\% & 96.68\% & 10.64\% & 4.07\% & 8.15(10.69)\\
% \dfjnewprapr & 1826 & 79 & 4 & 79 & 95.85\% & 95.85\% & 4.82\% & 5.04\% & 7.15(9.64)\\
% \dfjmerge & 2250 & 239 & 32 & 239 & 90.40\% & 90.40\% & 11.81\% & 15.29\% & 7(12.87)\\
% \dfjbalance & 120 & 151 & 120 & 151 & 44.28\% & 44.28\% & 44.28\% & 51.15\% & -\\
% \bottomrule
% \end{tabular}
% \label{tab:s3_performance}

\begin{tabular}{l|r|r|r|r|r|r|r|r|r}
\toprule
S3 & \textit{TP} & \textit{FP} & \textit{TN} & \textit{FN} & \textit{\overfitprecision} & \textit{\overfitrecall} & \textit{\correctrecall} & \textit{\prauc} & \textit{\avr}\\
\midrule
\shangwendata & 517 & 137 & 111 & 137 & 79.1\% & 79.1\% & 44.8\% & 45.3\% & 2.8(9.1)\\
\dfjoldprapr & 1222 & 42 & 5 & 42 & 96.7\% & 96.7\% & 10.6\% & 4.1\% & 8.2(10.7)\\
\dfjnewprapr & 1826 & 79 & 4 & 79 & 95.9\% & 95.9\% & 4.8\% & 5.0\% & 7.2(9.6)\\
\dfjmerge & 2250 & 239 & 32 & 239 & 90.4\% & 90.4\% & 11.8\% & 15.3\% & 7.0(12.9)\\
\dfjbalance & 120 & 151 & 120 & 151 & 44.3\% & 44.3\% & 44.3\% & 51.1\% & -\\
\bottomrule
\end{tabular}
\label{tab:s3_performance}

==> Tables/ssFix_performance.tex <==
% \begin{tabular}{l|r|r|r|r|r|r|r|r|r}
% \toprule
% ssFix & \textit{TP} & \textit{FP} & \textit{TN} & \textit{FN} & \textit{precision} & \textit{recall} & \textit{\correctrecall} & \textit{AUC} & \textit{AVR}\\
% \midrule
% \shangwendata & 515 & 139 & 109 & 139 & 78.75\% & 78.75\% & 43.95\% & 60.61\% & 2.72(9.1)\\
% \dfjoldprapr & 1,221 & 43 & 4 & 43 & 96.60\% & 96.60\% & 8.51\% & 49.50\% & 6.77(10.69)\\
% \dfjnewprapr & 1,826 & 79 & 4 & 79 & 95.85\% & 95.85\% & 4.82\% & 45.23\% & 6.26(9.64)\\
% \dfjmerge & 2,242 & 247 & 24 & 247 & 90.08\% & 90.08\% & 8.86\% & 45.46\% & 6.12(12.87)\\
% \dfjbalance & 129 & 142 & 129 & 142 & 47.60\% & 47.60\% & 47.60\% & 46.28\% & -\\
% \bottomrule
% \end{tabular}
% \label{tab:ssFix_performance}

% \begin{tabular}{l|r|r|r|r|r|r|r|r|r}
% \toprule
% ssFix & \textit{TP} & \textit{FP} & \textit{TN} & \textit{FN} & \textit{precision} & \textit{recall} & \textit{\correctrecall} & \textit{AUC} & \textit{AVR}\\
% \midrule
% \shangwendata & 515 & 139 & 109 & 139 & 78.75\% & 78.75\% & 43.95\% & 60.61\% & 2.72(9.1)\\
% \dfjoldprapr & 1221 & 43 & 4 & 43 & 96.60\% & 96.60\% & 8.51\% & 49.50\% & 6.77(10.69)\\
% \dfjnewprapr & 1826 & 79 & 4 & 79 & 95.85\% & 95.85\% & 4.82\% & 45.23\% & 6.26(9.64)\\
% \dfjmerge & 2242 & 247 & 24 & 247 & 90.08\% & 90.08\% & 8.86\% & 45.46\% & 6.12(12.87)\\
% \dfjbalance & 126 & 145 & 126 & 145 & 46.49\% & 46.49\% & 46.49\% & 45.88\% & -\\
% \bottomrule
% \end{tabular}
% \label{tab:ssFix_performance}

% \begin{tabular}{l|r|r|r|r|r|r|r|r|r}
% \toprule
% ssFix & \textit{TP} & \textit{FP} & \textit{TN} & \textit{FN} & \textit{precision} & \textit{recall} & \textit{\correctrecall} & \textit{PR-AUC} & \textit{AVR}\\
% \midrule
% \shangwendata & 515 & 139 & 109 & 139 & 78.75\% & 78.75\% & 43.95\% & 43.81\% & 2.72(9.1)\\
% \dfjoldprapr & 1221 & 43 & 4 & 43 & 96.60\% & 96.60\% & 8.51\% & 8.73\% & 6.77(10.69)\\
% \dfjnewprapr & 1826 & 79 & 4 & 79 & 95.85\% & 95.85\% & 4.82\% & 6.65\% & 6.26(9.64)\\
% \dfjmerge & 2242 & 247 & 24 & 247 & 90.08\% & 90.08\% & 8.86\% & 10.07\% & 6.12(12.87)\\
% \dfjbalance & 126 & 145 & 126 & 145 & 46.49\% & 46.49\% & 46.49\% & 48.29\% & -\\
% \bottomrule
% \end{tabular}
% \label{tab:ssFix_performance}

\begin{tabular}{l|r|r|r|r|r|r|r|r|r}
\toprule
ssFix & \textit{TP} & \textit{FP} & \textit{TN} & \textit{FN} & \textit{\overfitprecision} & \textit{\overfitrecall} & \textit{\correctrecall} & \textit{\prauc} & \textit{\avr}\\
\midrule
\shangwendata & 515 & 139 & 109 & 139 & 78.7\% & 78.7\% & 44.0\% & 43.8\% & 2.7(9.1)\\
\dfjoldprapr & 1221 & 43 & 4 & 43 & 96.6\% & 96.6\% & 8.5\% & 8.7\% & 6.8(10.7)\\
\dfjnewprapr & 1826 & 79 & 4 & 79 & 95.9\% & 95.9\% & 4.8\% & 6.7\% & 6.3(9.6)\\
\dfjmerge & 2242 & 247 & 24 & 247 & 90.1\% & 90.1\% & 8.9\% & 10.1\% & 6.1(12.9)\\
\dfjbalance & 126 & 145 & 126 & 145 & 46.5\% & 46.5\% & 46.5\% & 48.3\% & -\\
\bottomrule
\end{tabular}
\label{tab:ssFix_performance}

==> sections/Discussion.tex <==
\section{Discussion}
\Comment{Discuss the guidelines for future patch correctness checking and program repair in general.\\
\jun{I think we already have some results: 1. similarity based techniques are not working (including three static features and embedding); 2. although dynamic technique can achieve high precision, the recall is too low (if you only identify 10\% of overfitting patches, you still need to manually check the remaining 90\% patches, which means that's useless) 3. when using dynamic techniques, when generating tests, false positive tests and flaky tests could affect the performance of techniques. While removing those tests could be time consuming, not to mention dynamic techniques themselves cost a lot of time.}}
\jun{\textbf{Guidelines for \pcc.} Overall the direction of \pcc can be classified into \textit{dynamic techniques} and \textit{static techniques}. Dynamic techniques are based on the assumption that patch overfitting is the result of test suite inadequacy so the direction of dynamic techniques is to leverage more advanced test generation techniques to enhance test suite and filter out more overfitting patches. However, the limitations are two-fold: test generation is often expensive, and false positives are unavoidable when the oracle is missing. Static techniques (and learning-based ones) extract static features and predict patch correctness with specific heuristics. However, the heuristics summarized by researchers could be overfitting to specific datasets (like code similarity and ODS features). Code naturalness is currently the only heuristics that has stable performance in all datasets, suggesting that it could be a promising future direction for \pcc.}

\jun{\textbf{Evaluation metrics.} In this paper we follow the experiment settings of previous study~\cite{DBLP:conf/kbse/WangWLWQZMJ20} for most experiments. But this metrics may not be beneficial for future study. For one thing, as LLM becomes more and more dominant in repair community~\cite{xia2022practical}, there will be large amount of patches even for a single bug from a single tool, so the practical and fair metric is the ranking of correct patch for each bug instead of comparing patches accross different bugs. For another, in the future the patch datasets will be more imbalanced, because the number of semantically correct patches will be limited but the number of overfitting patches will grow significantly. Therefore the metrics like precision and recall will be invalid and meanningless.}

==> sections/rq4.tex <==
%\subsection{RQ4} ~\label{sec:rq4}

% We are surprised to find that Opad shows best performance in terms of precision.
% Besides, we are also curious why there are still some false positives, i.e., correct patches that are identified as overfitting.
% To mitigate the threat that our correct patches are too less compared with overfitting patches, we run combine our dataset with developer patches, i.e., 395 developer patches from \dfj 1.2 programs and \dfj 2.0 additional programs.
% However, when combined with developer patches, the performance of Opad significantly degrades.
% \begin{listing}
%         \inputminted[]{java}{listings/JacksonDatabind-102-mutant-1.src.patch}
%         
%         \caption{A developer patch identified as overfitting by Opad}
%         \label{lst:Opad_dev_false_positive_patch}
% \end{listing}
% \begin{listing}
%         \inputminted[]{java}{listings/JacksonDatabind-method.java}
%         
%         \caption{Method StdSerializer.findFormatOverrides}
%         \label{lst:Opad_dev_patch_method}
% \end{listing}
% Listing ~\ref{lst:Opad_dev_false_positive_patch} shows a developer patch that is identified as overfitting.
% This patch removes a \textit{if} check for \textit{property}.
% However, Opad is based on tests generated on original buggy programs, not aware of such semantic changes.
% When stepping into the method \textit{findFormatOverrides}~\ref{lst:Opad_dev_patch_method}, both \textit{provider} and \textit{prop} are null, leading to a \textit{NullPointerException}.
% The result is shown in \jun{google sheet}.
% Based on such observation and previous finding that developer patches often have greater modifications compared with \prapr patches, we hypothesis that developer patches could introduce not only bug-fixing modifications, but also some refactoring or semantics changes.
% Such changes could mislead Opad: Opad tests are generated on buggy programs and unaware of change of semantics, which could lead to some test failures on patched programs, especially when the difference is large.
% % To verify that, we explore the relation between scores of similarity-based techniques and whether a patch was wrongly classified as overfitting.
% \jun{To complete later.}
\subsection{RQ4: Entropy-based techniques} ~\label{sec:rq4}
\begin{table}[h]
  \setlength\tabcolsep{4.0pt} % horizental space
  \def\arraystretch{1.0}
  \scriptsize
  \caption{Performance of code naturalness}
  \centering
  \input{Tables/entropy_rank}
  \label{tab:entropy_rank}
  
\end{table}
\begin{table}[h]
  \setlength\tabcolsep{4.0pt} % horizental space
  \def\arraystretch{1.0}
  \scriptsize
  \caption{Average scores based on entropy}
  \centering
  \input{Tables/entropy_average}
  \label{tab:entropy_average}
  
\end{table}

As shown in Table\ref{tab:entropy_rank}, in all datasets (except \dfjbalance where AVR is not applicable) both \sumentropy and \meanentropy can outperform all three static techniques. Specifically, in terms of AVRs, the sum/mean entropy outperforms the best-performed static technique by 11.21\%/11.21\% (on \shangwendata), 30.13\%/31.31\%(on \dfjoldprapr), 34.82\%/25.40\%(on \dfjnewprapr), and 44.08\%/36.79\%(on \dfjmerge). Interestingly, our results also confirm prior work~\cite{xia2022practical} that \sumentropy performs slightly better than \meanentropy for PCC. The reason is that \sumentropy calculates the entire
sequence entropy for code naturalness computation, and considers both code naturalness and length information.\Comment{ thus shorter sequences tend to get lower naturalness, which is consistent with traditional static techniques~\cite{cite s3, capgen, etc} (which also favor simple patches over
complicated ones).}\Comment{relatively 11.21\% and 11.21\%(on \shangwendata), 30.13\% and 31.31\%(on \dfjoldprapr), 34.82\% and 25.40\%(on \dfjnewprapr), 44.08\% and 36.79\%(on \dfjmerge) higher than the best-performed static techniques.} 
\lingming{I cannot quite follow the following text, and am not sure if table 16 and the following text are helpful. given we are running out of space, can we remove them and merge this rq into rq1? }\jun{I agree}
% To further understand how naturalness can help distinguish overfitting patches and correct patches, we calculate the mean value of overfitting and correct patches in different datasets as shown in \ref{tab:entropy_average} and conduct a Mann-Whitney U Test to validate that. It shows that in all datasets both \sumentropy and \meanentropy of correct patches are significantly lower than overfitting patches. 
% Meanwhile, we also observe that the \avr on \prapr patches is lower than \shangwendata and the difference of mean value of entropy for overfitting and correct patches is smaller as well, 
In conclusion, entropy-based techniques show greater potential in \pcc and this is the first, to the best of our knowledge, evaluation of entropy-based techniques on \pcc datasets and we appeal to the community that more attention should be drawn into this direction.
\finding {Entropy-based techniques can beat all static techniques, and we find that correct patches have higher code naturalness than  overfitting patches.}
